Generalised Unsupervised Domain Adaptation of Neural Machine Translation with Cross-Lingual Data Selection

This paper considers the unsupervised domain adaptation problem for neural machine translation (NMT), where we assume the access to only monolingual text in either the source or target language in the new domain. We propose a cross-lingual data selection method to extract in-domain sentences in the missing language side from a large generic monolingual corpus. Our proposed method trains an adaptive layer on top of multilingual BERT by contrastive learning to align the representation between the source and target language. This then enables the transferability of the domain classifier between the languages in a zero-shot manner. Once the in-domain data is detected by the classifier, the NMT model is then adapted to the new domain by jointly learning translation and domain discrimination tasks. We evaluate our cross-lingual data selection method on NMT across five diverse domains in three language pairs, as well as a real-world scenario of translation for COVID-19. The results show that our proposed method outperforms other selection baselines up to +1.5 BLEU score.

==> sec2-backup2.tex <==
\section{Generalised Unsupervised Domain Adaptation}
%In this section, we first introduce the unknown domain adaptation problem, then discuss its challenge and the existing approaches in the literature to handle the problem.

% Domain adaptation is an important problem in NMT because it is very expensive to obtain training data that are both large and relevant to the test domain. Supervised adaptation problem requires the existence of OOD bitext and in-domain bitext. Unsupervised domain adaptation problem assumes OOD bitext and in-domain monotext, usually in target language.


A domain is defined as a distribution $P^{s,t}(X,Y)$ where $X$ are sequences in the \emph{source} language $s$ and $Y$ are corresponding translations in the \emph{target} language $t$.%
%
To avoid confusion with the terminologies  of source domain and target domain commonly used in the domain adaptation literature~\citep{uda-survey}, 
We denote the NMT domain \emph{prior} to the adaption stage by $P_{old}^{s,t}(X,Y)$; and subsequently $P_{new}^{s,t}(X,Y)$ our newly adapted NMT domain. 
%We note here that 
The source and target languages $s$ and $t$ are usually the same in the adaptation process, hence  we  drop superscript for brevity. % when the context is clear.


We define the generalised unsupervised domain adaptation (\guda)
%unknown domain adaptation (\textsc{UnkDA}) 
of NMT as the problem of adapting an NMT model trained on an old domain $P_{old}^{s,t}(X,Y)$ to a new domain $P_{new}^{s,t}(X,Y)$ where only \emph{either} the source $s$ or target $t$ monolingual language data is available in the new domain. 
Since $P^{s,t}(X,Y) = P^s(X)P^{s,t}(Y|X)$, therefore $P^s_{old}(X)$ is the distribution over sequences on the source language $s$ in the old domain and it is usually much richer (i.e., containing diverse categories such as news, politics) than  $P^s_{new}(X)$ which is typically a much more specific category where we aim to adapt NMT model\footnote{hence, our setting might also bear some similarity to knowledge distillation literature.}. The conditional distribution $P^{s,t}_{old}(Y|X)$ specify the encoding-decoding NMT network to be adapted to the new domain.

%its nature is unknown.
More specifically, given parallel bitext $\Dold:=\{(\vx_i,\vy_i)\}$ in the old domain, we consider two settings in the new domain where we have
\begin{itemize}[noitemsep,topsep=0pt]
    \item an initial source language monolingual text $\Xnew:=\{\vx_j\}$ and a  \emph{generic} monolingual text in the target language $\DT$.
    % we further assume the availability of a  \emph{generic} monolingual text in the target language $\DT$. 
    \item an initial target language monolingual text $\Ynew :=\{\vy_k\}$ and a  \emph{generic} monolingual text in the source language $\DS$.
    % we assume the availability  of a  \emph{generic} monolingual text in the source language $\DS$.
\end{itemize}
However, it is important to note that in both cases we {\bf do not} require any parallel text in the new domain, hence the term \emph{unsupervised domain adaptation} and the goal is to adapt an NMT model, parameterized by $\pmb{\theta}$, trained on the old domain  bitext $\Dold$ to the new domain. 

% \rodo{mention the usual formulation (using the target language in-domain monotex) is a special case of our formulation, which is widely used in the literature. mention that that the formulation involving the source in-domain monotext is not well explored in the literature. }

In the later setting, the text $\Ynew$ can be used to create pseudo-parallel data via back-translation \cite{sennrich-etal-2016-improving}, or to adapt the decoder via multi-task learning with language modelling objective \cite{gulcehre2015using,domhan-hieber-2017-using}. This setting is the usual formulation of most previous works in UDA for NMT~\cite{chu-wang-2018-survey}. In contrast, the setting involving the source monotext  $\Xnew$ is not well explored in the literature.

Our approach to address \guda is to create \emph{in-domain} monotext for the language side in the new domain for which we are not given. That is, if we are given $\Xnew$, we build a classifier to select monotext $\Ynew$ in the target language from the generic monotext $\DT$, and vice versa. 
%Similarly, if we are given $\Ynew$, we create in-domain monotext $\Xnew$ in the source language using the generic monotext $\DS$. 
%
We then adapt the NMT model based on the bitext from the old domain as well as the source and target language monotext in the new domain. 
%
The challenge, however, is how to train a classifier for data selection for the language-side with missing data.  
%
We address this problem in Section~\ref{sec:dataselection},  then mention how to adapt the NMT model to the new domain in Section~\ref{sec:uda-nmt}.


%\rodo{mention our approach: we do cross-lingual data retrieval to create in-domain monotext for the language side for which we are not given in-domain monotext. that is, if we are given which is missin}

%$\mathcal{D}_N$, and large general monolingual corpus $\mathcal{D}_S$ or $\mathcal{D}_T$ in source and target languages respectively. The goal is to have an NMT model to work well on the new domain $\mathcal{D}_N$.
%
%an NMT model parameterized by $\theta$ trained on parallel text $\mathcal{D}_{\textrm{old}}:=\{(\vx_i,\vy_i)\}$ in the old domain $\mathcal{D}_O$, a small initial monolingual text $\vX_N$ or $\vY_N$ from a new domain $\mathcal{D}_N$, and large monolingual corpus $\mathcal{D}_S$, $\mathcal{D}_T$ in source and target languages respectively. The goal is to have an NMT model to work well on the new domain $\mathcal{D}_N$.

%The main challenge of \textsc{UnkDA} is that the model designers do not know the nature of the domain in advance so that they can take advantage of the available in-domain monolingual data. \todo{elaborate more about the challenge}

%Depending on the assumption of the monotext in the new domain, \textsc{UnkDA} can be classified into three scenarios, which are non-parallel text from both source and target languages, only in-domain source language text, and only in-domain target language text. While the first two scenarios are the frequent assumptions of most previous works in domain adaption literature, very little attention has been paid to the only source-language in-domain text scenario. 

%The problem where there is no in-domain parallel data available, is also referred to as unsupervised domain adaptation and has been well-studied in the literature~\cite{chu-wang-2018-survey}. When only target side monolingual data is available, the text can be used to create pseudo-parallel corpus via back-translation \cite{sennrich-etal-2016-improving}, or to adapt the decoder via multi-task learning with language modelling objective \cite{gulcehre2015using,domhan-hieber-2017-using}.
%\todo{Previous works use only source-side}


% \begin{itemize}
%     \item Monolingual from source language: fewer study
%     \item Monolingual from target language: most UDA works \citep{dou-etal-2019-unsupervised}
% \end{itemize}


==> tab-seed-size.tex <==
\begin{table}[!h]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{l||rrr|rrr}
\toprule
 & \multicolumn{3}{c|}{law} & \multicolumn{3}{|c}{ted}\\
\multicolumn{1}{c||}{} & 
\multicolumn{1}{c}{10K} & \multicolumn{1}{c}{50K} & \multicolumn{1}{c|}{100K}
& \multicolumn{1}{c}{10K} & \multicolumn{1}{c}{50K} & \multicolumn{1}{c}{100K}
\\
\midrule
random &  \\
% n-gram & \\
CED &  \\
domain-finetune & \\
constrastive &  \\ 
\bottomrule
\end{tabular}
}
\caption{Result at various in-domain seed}
\label{tab:seed-size}
\end{center}
\end{table}

==> tab-selection-size.tex <==
\begin{table}[!h]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{l||rrr|rrr}
\toprule
 & \multicolumn{3}{c|}{law} & \multicolumn{3}{|c}{ted}\\
\multicolumn{1}{c||}{} & 
\multicolumn{1}{c}{10K} & \multicolumn{1}{c}{100K} & \multicolumn{1}{c|}{1M}
& \multicolumn{1}{c}{10K} & \multicolumn{1}{c}{10K} & \multicolumn{1}{c}{1M}
\\
\midrule
random &  \\
% n-gram & \\
CED &  \\
domain-finetune & \\
constrastive &  \\ 
\bottomrule
\end{tabular}
}
\caption{Result at various selection size}
\label{tab:selection-size}
\end{center}
\end{table}
